CrossOver: 3D Scene Cross-Modal Alignment

Multi-modal 3D object understanding has gained significant attention, yet current approaches often assume complete data availability and rigid alignment across all modalities. We present CrossOver, a novel framework for cross-modal 3D scene understanding via flexible, scene-level modality alignment. Unlike traditional methods that require aligned modality data for every object instance, CrossOver learns a unified, modality-agnostic embedding space for scenes by aligning modalities -- RGB images, point clouds, CAD models, floorplans, and text descriptions -- with relaxed constraints and without explicit object semantics. Leveraging dimensionality-specific encoders, a multi-stage training pipeline, and emergent cross-modal behaviors, CrossOver supports robust scene retrieval and object localization, even with missing modalities. Evaluations on ScanNet and 3RScan datasets show its superior performance across diverse metrics, highlighting the adaptability for real-world applications in 3D scene understanding.

==> tab/scan3r_combination_crossmodal_scene_retrieval.tex <==
\begin{table}[t]
  \centering
  \resizebox{\textwidth}{!}{
   \begin{tabular}{l| cccc | ccc}
    \toprule
    \textbf{Method} & \multicolumn{4}{c}{\textbf{Scene Matching Recall}  $\uparrow$} & \multicolumn{3}{c}{\textbf{Temporal Recall} $\uparrow$} \\
    \midrule\arrayrulecolor{black} 
    & \textbf{top-1} & \textbf{top-5} & \textbf{top-10} & \textbf{top-20} & \textbf{top-1} & \textbf{top-5} & \textbf{top-10} &
    \midrule\arrayrulecolor{black}
    \multicolumn{8}{l}{\cellcolor[HTML]{EEEEEE}{\textit{$\mathcal{I} + \mathcal{R} \rightarrow \mathcal{P}$}}} \\
    ULIP-2~\cite{xue2023ulip2} & 0.68 & 2.7 & 7.43 & 11.49 & 0 & 6.38 & 12.77 \\
    PointBind~\cite{pointbind} & 1.35 & 3.38 & 6.76 & 12.84 & 2.13 & 6.38 & 8.51 \\
    Inst.\ Baseline (Ours) & \nd6.08 & \nd24.32 & \nd39.19 & \nd56.08 & \nd6.38 & \nd25.53 & \nd38.3 \\
    Ours & \fs16.22 & \fs49.32 & \fs68.92 & \fs83.11 & \fs12.77 & \fs48.94 & \fs80.85 \\
    \hdashline 
    \multicolumn{8}{l}{\cellcolor[HTML]{EEEEEE}{\textit{$\mathcal{P} + \mathcal{R} \rightarrow \mathcal{I}$}}} \\
    ULIP-2~\cite{xue2023ulip2} & 1.35 & 5.41 & 8.78 & 15.54 & 2.13 & 8.51 & 14.89 \\
    PointBind~\cite{pointbind} & 1.35 & 5.41 & 8.78 & 16.22 & 2.13 & 10.64 & 19.15 \\
    Inst.\ Baseline (Ours) & \nd16.89 & \nd50.68 & \fs71.62 & \fs91.89 & \fs10.64 & \nd31.91 & \nd68.09 \\
    Ours & \fs19.59 & \fs51.35 & 65.54 & 85.81 & \nd8.51 & \fs34.04 & \fs70.21 \\
     
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Cross-Modal Combination Scene Retrieval on \textit{3RScan}.}}
    \label{tab:cross_modal_combination_scene_retrieval_scan3r}
\end{table}

==> tab/scannet_combination_crossmodal_scene_retrieval.tex <==
\begin{table*}[t]
  \centering
  \resizebox{\textwidth}{!}{
   \begin{tabular}{l| cccc | ccc| ccc || ccc}
    \toprule
    \textbf{Method} & \multicolumn{4}{c}{\textbf{Scene Matching Recall}  $\uparrow$} & \multicolumn{3}{c}{\textbf{Scene Category Recall} $\uparrow$} & \multicolumn{3}{c}{\textbf{Temporal Recall} $\uparrow$} & \multicolumn{3}{c}{\textbf{Intra-Category Recall} $\uparrow$} \\
    \midrule\arrayrulecolor{black} 
    & \textbf{top-1} & \textbf{top-5} & \textbf{top-10} & \textbf{top-20} & \textbf{top-1} & \textbf{top-5} & \textbf{top-10} &
    \textbf{top-1} & \textbf{top-5} & \textbf{top-10} &
    \textbf{top-1} & \textbf{top-3} & \textbf{top-5} \\
    \midrule\arrayrulecolor{black}
    \multicolumn{14}{l}{\cellcolor[HTML]{EEEEEE}{\textit{$\mathcal{I} + \mathcal{R} \rightarrow \mathcal{P}$}}} \\
    ULIP-2~\cite{xue2023ulip2} & 0.35 & 1.05 & 2.81 & 5.26 & 7.37 & 16.84 & 31.23 & 0 & 2.06 & 2.06 & 19.63 & 42.06 & 53.55 \\
    PointBind~\cite{pointbind} & 0.35 & 2.11 & 2.81 & 7.37 & 17.89 & 51.93 & 60.35 & 0 & 2.06 & 3.09 & 18.9 & 43.78 & 58.15 \\
    Inst.\ Baseline (Ours) & \nd7.39 & \nd37.32 & \nd55.99 & \nd72.89 & \nd38.03 & \nd75 & \nd86.62 & \nd11.34 & \nd36.08 & \nd55.67 & \nd36.65 & \nd72.87 & \fs85.36 \\
    Ours & \fs 18.25 & \fs 56.49 & \fs73.33 & \fs88.42 & \fs69.82 & \fs89.82 & \fs92.63 & \fs15.46 & \fs40.21 & \fs69.07 & \fs38.59 & \fs75.08 & \nd83.28 \\
    \hdashline
     \multicolumn{14}{l}{\cellcolor[HTML]{EEEEEE}{\textit{$\mathcal{P} + \mathcal{R} \rightarrow \mathcal{I}$}}} \\
     ULIP-2~\cite{xue2023ulip2} & 2.81 & 7.72 & 14.39 & 19.65 & 11.58 & 43.86 & 55.44 & 1.03 & 4.12 & 11.34 & 24.47 & 46.43 & 59.96 \\
     PointBind~\cite{pointbind} & 1.05 & 7.02 & 12.63 & 20 & 24.21 & 30.53 & 45.26 & 1.03 & 4.12 & 12.37 & 24.21 & 30.53 & 45.26 \\
     Inst.\ Baseline (Ours)& \nd19.72 & \nd60.92 & \nd75 & \nd87.68 & \nd66.2 & \fs87.68 & \fs94.01 & \fs12.37 & \nd40.21 & \nd70.1 & \fs46.56 & \nd76.31 & \nd86.94 \\
     Ours & \fs20.7 & \fs62.81 & \fs77.89 & \fs88.77 & \fs72.28 & \nd85.26 & \nd92.98 & \nd7.22 & \fs44.33 & \fs75.26 & \nd41.96 & \fs80.96 & \fs90.2 \\
     \midrule
     \midrule
     \multicolumn{14}{l}{\cellcolor[HTML]{EEEEEE}{\textit{$\mathcal{P} + \mathcal{R} \rightarrow \mathcal{F}$}}} \\
     ULIP-2~\cite{xue2023ulip2} & \nd0.7 & \nd3.16 & \nd5.26 & 8.77 & 8.07 & \nd43.86 & 48.07 & 0 & \nd5.15 & 7.22 & \nd16.43 & 39.89 & 55.85 \\
    PointBind~\cite{pointbind} & 0.35 & 1.75 & 3.86 & \nd9.12 & \nd14.74 & 27.02 & \nd48.42 & \nd1.03 & \nd5.15 & \nd8.25 & 13.82 & \nd39.93 & \nd57.71 \\
    Ours & \fs10.18 & \fs33.33 & \fs50.53 & \fs70.18 & \fs56.49 & \fs78.95 & \fs85.96 & \fs12.37 & \fs31.96 & \fs56.7 & \fs33.87 & \fs65.56 & \fs77.71 \\
     \hdashline

     \multicolumn{14}{l}{\cellcolor[HTML]{EEEEEE}{\textit{$\mathcal{F} + \mathcal{R} \rightarrow \mathcal{P}$}}} \\
     ULIP-2~\cite{xue2023ulip2} & 0 & 1.75 & 2.81 & 5.26 & 7.37 & 28.07 & 50.53 & \nd1.03 & 1.03 & 2.06 & 15.49 & 39.7 & 55.98 \\
    PointBind~\cite{pointbind} & \nd0.35 & \nd1.75 & \nd2.81 & \nd6.67 & \nd17.89 & \nd52.63 & \nd60.35 & 0 & \nd2.06 & \nd3.09 & \nd18.9 & \nd43.27 & \nd58.77 \\
    Ours & \fs11.93 & \fs42.81 & \fs63.86 & \fs77.89 & \fs63.86 & \fs81.05 & \fs88.77 & \fs11.34 & \fs31.96 & \fs59.79 & \fs31.56 & \fs66.84 & \fs81.22 \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Cross-Modal Combination Scene Retrieval on \textit{ScanNet}.}}
    \label{tab:cross_modal_combination_scene_retrieval_scannet}
\end{table*}
